SDP Synthesis of Maximum Coverage Trees for Probabilistic Planning under Control Constraints

The paper presents Maximal Covariance Backward Reachable Trees (MAXCOVAR BRT), which is a multi-query algorithm for planning of dynamic systems under stochastic motion uncertainty and constraints on the control input with explicit coverage guarantees. In contrast to existing roadmap-based probabilistic planning methods that sample belief nodes randomly and draw edges between them \cite{csbrm_tro2024}, under control constraints, the reachability of belief nodes needs to be explicitly established and is determined by checking the feasibility of a non-convex program. Moreover, there is no explicit consideration of coverage of the roadmap while adding nodes and edges during the construction procedure for the existing methods. Our contribution is a novel optimization formulation to add nodes and construct the corresponding edge controllers such that the generated roadmap results in provably maximal coverage under control constraints as compared to any other method of adding nodes and edges. We characterize formally the notion of coverage of a roadmap in this stochastic domain via introduction of the h-$\operatorname{BRS}$ (Backward Reachable Set of Distributions) of a tree of distributions under control constraints, and also support our method with extensive simulations on a 6 DoF model.

==> analysis.tex <==
\section{Analysis}

==> notes.tex <==
\begin{comment}
    Things to say:
    \begin{itemize}
    1. In the absence of control constraints, all maneuvers are feasible.
    2. In our setting, control sequence exists only if the set of equations is consistent. 
    3. Define the following objects: k-backreach set for a certain goal distribution. An example of a distribution reaching the goal in 40 steps but not 20 steps. Give a simulation -> improves readability of the paper and gets across the idea smoothly.
    4. Feasibility checking scales with time horizon.
    5. Solution: Build a tree of distributions that are verified to reach the goal, and find a path to one of the nodes on the tree (recursive feasibility checking).
    \end{itemize}

    Other things to say:
    \begin{itemize}
    1. If paths from a max_covar are found; then paths from covar <= max_covar are already found -> re-use.
    2. Size of the goal uncertainty etc.
    3. CC-RRT BWilliams sample open-loop control actions which can't control the size of the covariance.
    \end{itemize}
\end{comment}

==> related_work.tex <==
\cblue{\bf{Start populating the bib file...}}
\begin{itemize}
    \item Stochastic Motion Planning: CC-RRT, Brian Williams
    \item POMDP: FIRM, CS-BRM $\rightarrow$ \textit{difference in our approach versus theirs is a discussion of coverage}. Other roadmap based POMDP solutions - IGRES and MIGS (https://arxiv.org/pdf/2011.03813.pdf). \cred{Understand this former stated statement deeply.} Verify $\rightarrow$ pending. General overview of use of macro-actions in POMDPs pending...
    \item LTL: New papers found (focus just on composition not on synthesis)
    \item Djorde Zikelic papers: Don't have control constraints
    \item State-space partitioning in (continuous action) MDPs. Also, the state abstraction stuff in MDPs $\rightarrow$ David Abel's thesis. Also study state aggregation for MDPs (my hunch is that transitions over these state-space partitions become non-Markov). How to handle nonlinear stochastic models $\rightarrow$ by approximating the model as an MDP? But how to generate that approximate MDP?
    \item Goal-reaching MDPs: Model-based, model-free...
\end{itemize}
